Predicting Human Translation Difficulty with Neural Machine Translation

Human translators linger on some words and phrases more than others, and predicting this variation is a step towards explaining the underlying cognitive processes. Using data from the CRITT Translation Process Research Database, we evaluate the extent to which surprisal and attentional features derived from a Neural Machine Translation (NMT) model account for reading and production times of human translators. We find that surprisal and attention are complementary predictors of translation difficulty, and that surprisal derived from a NMT model is the single most successful predictor of production duration. Our analyses draw on data from hundreds of translators operating across 13 language pairs, and represent the most comprehensive investigation of human translation difficulty to date.

==> tables/tab-att-features.tex <==
\begingroup
% \renewcommand{\arraystretch}{2}
\begin{table*}
\footnotesize
% \centering
\setlength{\tabcolsep}{8pt}
% \begin{subtable}{.6\textwidth}
\centering
\begin{tabular}{ccccc}
% \multicolumn{6}{l}{\makecell{Given a source sequence $\bs{u} = [u_0, ..., u_m]$ and a target
% sequence $\bs{v} = [v_0, ..., v_p]$}} \\
\toprule
% & & \multicolumn{5}{c}{$\rho \uparrow $} \\
 Prediction  &  \multicolumn{1}{c}{Encoder attention, $A^{\mathrm{e}}$ } & \multicolumn{1}{c}{Cross-attention, $A^{\mathrm{x}}$ } & \multicolumn{1}{c}{ Decoder attention, $A^{\mathrm{d}}$} \\
% \cmidrule(lr){2-7} 
\midrule
\noalign{\vskip 2mm} 
\shortstack{Reading time of \\ source text, $\bs{u}$} &  

 ${\begin{aligned}
    & a^{\mathrm{e}}_{u,u} = \mathrm{att}(A^{\mathrm{e}}, \bs{i}, \bs{i}) \label{eq:u2u} \\ 
    &a^{\mathrm{e}}_{u,\Tilde{u}} = \mathrm{att}(A^{\mathrm{e}}, \bs{i}, \bs{\Tilde{i}})  \\ 
    &a^{\mathrm{e}}_{u,\texttt{eos}} = \mathrm{att}(A^{\mathrm{e}}, \bs{i}, [i_{\texttt{eos}}]) \\ 
    & a^{\mathrm{e}}_{\Tilde{u},u} = \mathrm{att}(A^{\mathrm{e}}, \bs{\Tilde{i}}, \bs{i}) \\
    & H^{\mathrm{e}}_{u,x} = H(A^{\mathrm{e}}, \bs{i}, \bs{m}) \\
\end{aligned}} $
& 
 ${\begin{aligned}
& a^{\mathrm{x}}_{y,u} = \mathrm{att}(A^{\mathrm{x}}, \bs{n}, \bs{i}) \\
\end{aligned}} $
& 
 ---
\\ 

% \midrule 
\noalign{\vskip 2mm} 
\makecell{Reading time /\\ production duration  \\of target text, $\bs{v}$} &

---
& ${\begin{aligned}
&a^{\mathrm{x}}_{v,\texttt{eos}} = \mathrm{att}(A^{\mathrm{x}}, \bs{j}, [i_{\texttt{eos}}]) \\ 
& H^{\mathrm{x}}_{v,x} = H(A^{\mathrm{x}}, \bs{j}, \bs{m}) \\
\end{aligned}} $
&
 ${\begin{aligned}
    &a^{\mathrm{d}}_{v,v} = \mathrm{att}(A^{\mathrm{d}}, \bs{j}, \bs{j}) \\ 
    &a^{\mathrm{d}}_{v,\Tilde{v}} = \mathrm{att}(A^{\mathrm{d}}, \bs{j}, \bs{\Tilde{j}})  \\ 
    & H^{\mathrm{d}}_{v,\overleftarrow{v}}  = H(A^{\mathrm{d}}, \bs{j}, \bs{\Tilde{j}} \cup \bs{j}) \\
\end{aligned}} $

\\ 
\noalign{\vskip 2mm}  \midrule
\end{tabular}
\begin{tabular}{ll}
% &&& \\
\noalign{\vskip 2mm} 
\multicolumn{2}{l}{
 ${\begin{aligned}
&\mathrm{att}(A, \bs{k}, \bs{l}) = \sum\limits_{l \in \bs{l}} \sum\limits_{k \in \bs{k}}  \alpha_{kl} \quad \text{where} \:A\: \text{is an attention matrix, } \:\alpha_{kl}\: \text{is the attention directed from $k$ to $l$} \\
& H(A, \bs{k}, \bs{l}) = \sum\limits_{k \in \bs{k}} \sum\limits_{l \in \bs{l}} - \hat{\alpha}_{kl} \log \hat{\alpha}_{kl}  \ \, \text{where} \ \,
 \hat{\alpha}_{kl} = \frac{\alpha_{kl}}{\lVert \bs{\alpha}_{k\veryshortarrow\bs{l}} \rVert} \,\text{and $\bs{\alpha}_{k\veryshortarrow\bs{l}}$ is a vector from $k$ to indices $\bs{l}$}  \\ 
 \end{aligned}}$
}
 \\ \noalign{\vskip 2mm}
\multicolumn{2}{l}{
 ${\begin{aligned}
 &\text{source sequence:}\: \bs{x} = [x_1, ..., x_m] \:\text{, with token indices} \ \bs{m} = \{1,...,m\}\\
 & \text{segment of $\bs{x}$:}\: \bs{u} = \bs{x}_{\bs{i}}\; \text{, with token indices}\: \bs{i} \subseteq \bs{m}  \:\text{,}  \ \,  \text{context of $\bs{u}$: } \bs{\Tilde{u}} = \bs{y}_{\bs{\Tilde{i}}} \,\text{where indices} \: \bs{\Tilde{i}} = \bs{m} \setminus \bs{i} \\
 & i_{\texttt{eos}} = m+1 \:\text{, the index of input sequence \texttt{eos}}\\ 
  &\text{target sequence:}\: \bs{y} = [y_1, ..., y_n] \:\text{, with token indices} \ \bs{n} = \{1,...,n\}\\
 & \text{segment of $\bs{y}$:}\: \bs{v} = \bs{y}_{\bs{j}}\;\text{, with token indices}\: \bs{j} \subseteq \bs{n}  \:\text{,} \ \, \text{preceding context:}\: \bs{\Tilde{v}} =  \bs{y}_{\bs{\Tilde{j}}} \:\text{where}\: \bs{\Tilde{j}} = \{1, ..., \max(\bs{j})\} \setminus \bs{j}
 \end{aligned}}$
}

%  \\ \noalign{\vskip 2mm}     

% ${\begin{aligned}
%  &m+1 \: \text{is the index of} \\
%  & \text{\texttt{eos} token} \\
%  & \bs{p} = [0..p] \\
%  \end{aligned}}$ &  
 


 \\

\end{tabular}

\caption{Definitions of attentional features extracted from NMT encoder and decoder. We combine directed attentions by computing the sum ($\mathrm{att}$) or entropy ($H$). The features predict translation difficulty of any given source segment, $\bs{u}$, and target segment, $\bs{v}$. We interpret each feature in Section~\ref{sec:attention}.}
% \end{subtable}%
\label{tab:att-features}
\end{table*}
\endgroup
